The Delegation Divide: An Open Index of AI-Agent Delegability across Occupations and Countries

35.2% of task time in world employment is at least partly delegable to AI agents in 2026, and only 2.5% can be handed over in full. Existing measures score exposure to generative AI, mostly for the United States. We build the Agent Delegability Index (ADI): two language models rate all 18,796 O*NET 30.2 task statements on a frozen, preregistered rubric of delegation levels and barriers; tasks are mapped to 433 ISCO-08 unit groups and weighted by ILOSTAT employment in 146 countries. Four findings. First, delegable employment rises with income, from 22.5% in low-income to 48.7% in high-income countries, a slope of 7.23 percentage points per log point of GDP per capita. This delegation divide is compositional: the physical barrier dominates the jobs poorer countries employ most. Second, at the occupation level ADI tracks exposure closely (r = 0.93 with Eloundou et al. and 0.89 with Felten et al.), above the preregistered bound of 0.80; ADI adds delegation levels and barriers on top of exposure, for the world, not a new ranking of occupations. Third, full delegation is rare and peaks for tasks that take a human about twelve minutes (11.8 minutes). Fourth, the preregistered adoption gap is not supported: across 101 countries, delegability and observed AI usage correlate at r = 0.86, and the gap between them is not wider in middle-income countries (p = 0.27). Model agreement is kappa = 0.77; a blind human rating of 300 tasks agrees with the model consensus at kappa = 0.85, and an agentic panel with web search at kappa = 0.87. We release the index, the atlas, the prompts and an MCP server at https://github.com/Cespial/delegation-divide.

==> cifras.tex <==
% generado por articulo/generar_cifras.py desde salidas_diseno/claims_diseno.jsonl y salidas/claims.jsonl — no editar a mano
\makeatletter
\providecommand{\cifra}{}\providecommand{\cifraopc}{}\providecommand{\cifraabs}{}\providecommand{\pval}{}
\renewcommand{\cifra}[1]{\@ifundefined{cf@#1}{\textbf{??\detokenize{#1}}}{\@nameuse{cf@#1}}}
\renewcommand{\cifraopc}[1]{\@ifundefined{cf@#1}{--}{\@nameuse{cf@#1}}}
\renewcommand{\cifraabs}[1]{\@ifundefined{cfa@#1}{\textbf{??\detokenize{#1}}}{\@nameuse{cfa@#1}}}
\renewcommand{\pval}[1]{\@ifundefined{cfp@#1}{\textbf{??\detokenize{#1}}}{\@nameuse{cfp@#1}}}
\@namedef{cf@agree.alpha.humano.modelo}{0.88}
\@namedef{cfa@agree.alpha.humano.modelo}{0.88}
\@namedef{cf@agree.alpha.modelos}{0.75}
\@namedef{cfa@agree.alpha.modelos}{0.75}
\@namedef{cf@agree.alpha.panel.modelo}{0.88}
\@namedef{cfa@agree.alpha.panel.modelo}{0.88}
\@namedef{cf@agree.exacto.humano.modelo.pct}{71.0}
\@namedef{cfa@agree.exacto.humano.modelo.pct}{71.0}
\@namedef{cf@agree.exacto.panel.modelo.pct}{80.8}
\@namedef{cfa@agree.exacto.panel.modelo.pct}{80.8}
\@namedef{cf@agree.kappa.humano.haiku}{0.79}
\@namedef{cfa@agree.kappa.humano.haiku}{0.79}
\@namedef{cf@agree.kappa.humano.modelo}{0.85}
\@namedef{cfa@agree.kappa.humano.modelo}{0.85}
\@namedef{cf@agree.kappa.humano.sonnet}{0.85}
\@namedef{cfa@agree.kappa.humano.sonnet}{0.85}
\@namedef{cf@agree.kappa.panel.haiku}{0.81}
\@namedef{cfa@agree.kappa.panel.haiku}{0.81}
\@namedef{cf@agree.kappa.panel.humano}{0.86}
\@namedef{cfa@agree.kappa.panel.humano}{0.86}
\@namedef{cf@agree.kappa.panel.modelo}{0.87}
\@namedef{cfa@agree.kappa.panel.modelo}{0.87}
\@namedef{cf@agree.kappa.panel.sonnet}{0.88}
\@namedef{cfa@agree.kappa.panel.sonnet}{0.88}
\@namedef{cf@agree.kappa.sonnet_haiku}{0.77}
\@namedef{cfa@agree.kappa.sonnet_haiku}{0.77}
\@namedef{cf@agree.testretest.haiku.exacto.pct}{87.0}
\@namedef{cfa@agree.testretest.haiku.exacto.pct}{87.0}
\@namedef{cf@agree.testretest.haiku.kappa}{0.88}
\@namedef{cfa@agree.testretest.haiku.kappa}{0.88}
\@namedef{cf@agree.testretest.sonnet.exacto.pct}{95.0}
\@namedef{cfa@agree.testretest.sonnet.exacto.pct}{95.0}
\@namedef{cf@agree.testretest.sonnet.kappa}{0.97}
\@namedef{cfa@agree.testretest.sonnet.kappa}{0.97}
\@namedef{cf@cobertura.empleo_millones}{2,336.3}
\@namedef{cfa@cobertura.empleo_millones}{2,336.3}
\@namedef{cf@cobertura.geih.isco}{426}
\@namedef{cfa@cobertura.geih.isco}{426}
\@namedef{cf@cobertura.ingreso.alto.paises}{53}
\@namedef{cfa@cobertura.ingreso.alto.paises}{53}
\@namedef{cf@cobertura.ingreso.bajo.paises}{17}
\@namedef{cfa@cobertura.ingreso.bajo.paises}{17}
\@namedef{cf@cobertura.ingreso.medio_alto.paises}{43}
\@namedef{cfa@cobertura.ingreso.medio_alto.paises}{43}
\@namedef{cf@cobertura.ingreso.medio_bajo.paises}{33}
\@namedef{cfa@cobertura.ingreso.medio_bajo.paises}{33}
\@namedef{cf@cobertura.isco}{433}
\@namedef{cfa@cobertura.isco}{433}
\@namedef{cf@cobertura.isco.imputados}{7}
\@namedef{cfa@cobertura.isco.imputados}{7}
\@namedef{cf@cobertura.oes.isco}{432}
\@namedef{cfa@cobertura.oes.isco}{432}
\@namedef{cf@cobertura.paises}{146}
\@namedef{cfa@cobertura.paises}{146}
\@namedef{cf@cobertura.paises.1d}{20}
\@namedef{cfa@cobertura.paises.1d}{20}
\@namedef{cf@cobertura.paises.2d}{126}
\@namedef{cfa@cobertura.paises.2d}{126}
\@namedef{cf@cobertura.paises.sin_pib}{0}
\@namedef{cfa@cobertura.paises.sin_pib}{0}
\@namedef{cf@cobertura.tareas}{18,796}
\@namedef{cfa@cobertura.tareas}{18,796}
\@namedef{cf@cobertura.tareas.puntuadas}{18,796}
\@namedef{cfa@cobertura.tareas.puntuadas}{18,796}
\@namedef{cf@d3.h1.n}{150}
\@namedef{cfa@d3.h1.n}{150}
\@namedef{cf@d3.h1.pendiente.150}{7.30}
\@namedef{cfa@d3.h1.pendiente.150}{7.30}
\@namedef{cf@d3.n.paises}{150}
\@namedef{cfa@d3.n.paises}{150}
\@namedef{cf@d3.titular.l2.150}{35.20}
\@namedef{cfa@d3.titular.l2.150}{35.20}
\@namedef{cf@d3.titular.l2.con_regla}{35.17}
\@namedef{cfa@d3.titular.l2.con_regla}{35.17}
\@namedef{cf@diseno.agro.en_muestra}{193}
\@namedef{cfa@diseno.agro.en_muestra}{193}
\@namedef{cf@diseno.agro.tareas}{193}
\@namedef{cfa@diseno.agro.tareas}{193}
\@namedef{cf@diseno.atlas.paises}{146}
\@namedef{cfa@diseno.atlas.paises}{146}
\@namedef{cf@diseno.atlas.paises.1d}{20}
\@namedef{cfa@diseno.atlas.paises.1d}{20}
\@namedef{cf@diseno.atlas.paises.2d}{126}
\@namedef{cfa@diseno.atlas.paises.2d}{126}
\@namedef{cf@diseno.ibs.filas}{1,131}
\@namedef{cfa@diseno.ibs.filas}{1,131}
\@namedef{cf@diseno.ibs.isco}{436}
\@namedef{cfa@diseno.ibs.isco}{436}
\@namedef{cf@diseno.ibs.k1}{683}
\@namedef{cfa@diseno.ibs.k1}{683}
\@namedef{cf@diseno.ibs.k2}{102}
\@namedef{cfa@diseno.ibs.k2}{102}
\@namedef{cf@diseno.ibs.k3}{30}
\@namedef{cfa@diseno.ibs.k3}{30}
\@namedef{cf@diseno.ibs.k4mas}{24}
\@namedef{cfa@diseno.ibs.k4mas}{24}
\@namedef{cf@diseno.ibs.kmax}{17}
\@namedef{cfa@diseno.ibs.kmax}{17}
\@namedef{cf@diseno.ibs.soc}{839}
\@namedef{cfa@diseno.ibs.soc}{839}
\@namedef{cf@diseno.ilostat.paises.1d}{173}
\@namedef{cfa@diseno.ilostat.paises.1d}{173}
\@namedef{cf@diseno.ilostat.paises.1d.desde2019}{151}
\@namedef{cfa@diseno.ilostat.paises.1d.desde2019}{151}
\@namedef{cf@diseno.ilostat.paises.2d}{144}
\@namedef{cfa@diseno.ilostat.paises.2d}{144}
\@namedef{cf@diseno.ilostat.paises.2d.desde2019}{134}
\@namedef{cfa@diseno.ilostat.paises.2d.desde2019}{134}
\@namedef{cf@diseno.onet.ocupaciones}{923}
\@namedef{cfa@diseno.onet.ocupaciones}{923}
\@namedef{cf@diseno.onet.tareas}{18,796}
\@namedef{cfa@diseno.onet.tareas}{18,796}
\@namedef{cf@diseno.onet10_19.codigos2010}{1,110}
\@namedef{cfa@diseno.onet10_19.codigos2010}{1,110}
\@namedef{cf@diseno.onet10_19.codigos2019}{1,012}
\@namedef{cfa@diseno.onet10_19.codigos2019}{1,012}
\@namedef{cf@diseno.onet10_19.multiples}{97}
\@namedef{cfa@diseno.onet10_19.multiples}{97}
\@namedef{cf@diseno.piloto.envoltorio.kappa}{0.70}
\@namedef{cfa@diseno.piloto.envoltorio.kappa}{0.70}
\@namedef{cf@diseno.piloto.envoltorio.nivel}{1.64}
\@namedef{cfa@diseno.piloto.envoltorio.nivel}{1.64}
\@namedef{cf@diseno.piloto.lote.haiku.kappa}{0.56}
\@namedef{cfa@diseno.piloto.lote.haiku.kappa}{0.56}
\@namedef{cf@diseno.piloto.lote.sonnet.kappa}{0.60}
\@namedef{cfa@diseno.piloto.lote.sonnet.kappa}{0.60}
\@namedef{cf@diseno.piloto.lote.tareas}{25}
\@namedef{cfa@diseno.piloto.lote.tareas}{25}
\@namedef{cf@diseno.piloto.neutro.nivel}{1.33}
\@namedef{cfa@diseno.piloto.neutro.nivel}{1.33}
\@namedef{cf@diseno.previo.conjuntos}{9}
\@namedef{cfa@diseno.previo.conjuntos}{9}
\@namedef{cf@diseno.previo.ocupaciones}{440}
\@namedef{cfa@diseno.previo.ocupaciones}{440}
\@namedef{cf@diseno.previo.ocupaciones_por_tarea.mediana}{77}
\@namedef{cfa@diseno.previo.ocupaciones_por_tarea.mediana}{77}
\@namedef{cf@diseno.puente.conjuntos}{403}
\@namedef{cfa@diseno.puente.conjuntos}{403}
\@namedef{cf@diseno.puente.imputados}{7}
\@namedef{cfa@diseno.puente.imputados}{7}
\@namedef{cf@diseno.puente.isco}{433}
\@namedef{cfa@diseno.puente.isco}{433}
\@namedef{cf@diseno.puente.pares}{30,549}
\@namedef{cfa@diseno.puente.pares}{30,549}
\@namedef{cf@diseno.puente.tareas}{18,796}
\@namedef{cfa@diseno.puente.tareas}{18,796}
\@namedef{cf@diseno.puente.tareas_grupo.max}{860}
\@namedef{cfa@diseno.puente.tareas_grupo.max}{860}
\@namedef{cf@diseno.puente.tareas_grupo.mediana}{48}
\@namedef{cfa@diseno.puente.tareas_grupo.mediana}{48}
\@namedef{cf@diseno.puente.tareas_grupo.min}{5}
\@namedef{cfa@diseno.puente.tareas_grupo.min}{5}
\@namedef{cf@diseno.reps}{1,000}
\@namedef{cfa@diseno.reps}{1,000}
\@namedef{cf@diseno.semilla}{20,261,020}
\@namedef{cfa@diseno.semilla}{20,261,020}
\@namedef{cf@envoltorio.haiku.kappa}{0.76}
\@namedef{cfa@envoltorio.haiku.kappa}{0.76}
\@namedef{cf@envoltorio.haiku.kappa.humano.cc}{0.75}
\@namedef{cfa@envoltorio.haiku.kappa.humano.cc}{0.75}
\@namedef{cf@envoltorio.haiku.kappa.humano.neutro}{0.79}
\@namedef{cfa@envoltorio.haiku.kappa.humano.neutro}{0.79}
\@namedef{cf@envoltorio.haiku.l2.cc.pct}{56.2}
\@namedef{cfa@envoltorio.haiku.l2.cc.pct}{56.2}
\@namedef{cf@envoltorio.haiku.l2.neutro.pct}{54.9}
\@namedef{cfa@envoltorio.haiku.l2.neutro.pct}{54.9}
\@namedef{cf@envoltorio.haiku.n}{1,500}
\@namedef{cfa@envoltorio.haiku.n}{1,500}
\@namedef{cf@envoltorio.haiku.n.humano}{300}
\@namedef{cfa@envoltorio.haiku.n.humano}{300}
\@namedef{cf@envoltorio.haiku.nivel.cc}{1.40}
\@namedef{cfa@envoltorio.haiku.nivel.cc}{1.40}
\@namedef{cf@envoltorio.haiku.nivel.neutro}{1.36}
\@namedef{cfa@envoltorio.haiku.nivel.neutro}{1.36}
\@namedef{cf@envoltorio.sonnet.kappa}{0.60}
\@namedef{cfa@envoltorio.sonnet.kappa}{0.60}
\@namedef{cf@envoltorio.sonnet.kappa.humano.cc}{0.61}
\@namedef{cfa@envoltorio.sonnet.kappa.humano.cc}{0.61}
\@namedef{cf@envoltorio.sonnet.kappa.humano.neutro}{0.85}
\@namedef{cfa@envoltorio.sonnet.kappa.humano.neutro}{0.85}
\@namedef{cf@envoltorio.sonnet.l2.cc.pct}{56.8}
\@namedef{cfa@envoltorio.sonnet.l2.cc.pct}{56.8}
\@namedef{cf@envoltorio.sonnet.l2.neutro.pct}{37.6}
\@namedef{cfa@envoltorio.sonnet.l2.neutro.pct}{37.6}
\@namedef{cf@envoltorio.sonnet.n}{1,500}
\@namedef{cfa@envoltorio.sonnet.n}{1,500}
\@namedef{cf@envoltorio.sonnet.n.humano}{300}
\@namedef{cfa@envoltorio.sonnet.n.humano}{300}
\@namedef{cf@envoltorio.sonnet.nivel.cc}{1.53}
\@namedef{cfa@envoltorio.sonnet.nivel.cc}{1.53}
\@namedef{cf@envoltorio.sonnet.nivel.neutro}{1.04}
\@namedef{cfa@envoltorio.sonnet.nivel.neutro}{1.04}
\@namedef{cf@extremo.isco.bot1.id}{9121}
\@namedef{cf@extremo.isco.bot1.l2}{0.0}
\@namedef{cfa@extremo.isco.bot1.l2}{0.0}
\@namedef{cf@extremo.isco.bot1.nombre}{hand launderers and pressers}
\@namedef{cf@extremo.isco.bot2.id}{9312}
\@namedef{cf@extremo.isco.bot2.l2}{0.0}
\@namedef{cfa@extremo.isco.bot2.l2}{0.0}
\@namedef{cf@extremo.isco.bot2.nombre}{civil engineering labourers}
\@namedef{cf@extremo.isco.bot3.id}{9311}
\@namedef{cf@extremo.isco.bot3.l2}{0.0}
\@namedef{cfa@extremo.isco.bot3.l2}{0.0}
\@namedef{cf@extremo.isco.bot3.nombre}{mining and quarrying labourers}
\@namedef{cf@extremo.isco.n.max}{13}
\@namedef{cfa@extremo.isco.n.max}{13}
\@namedef{cf@extremo.isco.n.min}{16}
\@namedef{cfa@extremo.isco.n.min}{16}
\@namedef{cf@extremo.isco.top1.id}{4413}
\@namedef{cf@extremo.isco.top1.l2}{100.0}
\@namedef{cfa@extremo.isco.top1.l2}{100.0}
\@namedef{cf@extremo.isco.top1.nombre}{coding, proof-reading and related clerks}
\@namedef{cf@extremo.isco.top2.id}{5244}
\@namedef{cf@extremo.isco.top2.l2}{100.0}
\@namedef{cfa@extremo.isco.top2.l2}{100.0}
\@namedef{cf@extremo.isco.top2.nombre}{contact centre salespersons}
\@namedef{cf@extremo.isco.top3.id}{4419}
\@namedef{cf@extremo.isco.top3.l2}{100.0}
\@namedef{cfa@extremo.isco.top3.l2}{100.0}
\@namedef{cf@extremo.isco.top3.nombre}{clerical support workers not elsewhere classified}
\@namedef{cf@extremo.pais.bot1.id}{BDI}
\@namedef{cf@extremo.pais.bot1.l2}{14.7}
\@namedef{cfa@extremo.pais.bot1.l2}{14.7}
\@namedef{cf@extremo.pais.bot1.nombre}{Burundi}
\@namedef{cf@extremo.pais.bot2.id}{MOZ}
\@namedef{cf@extremo.pais.bot2.l2}{17.9}
\@namedef{cfa@extremo.pais.bot2.l2}{17.9}
\@namedef{cf@extremo.pais.bot2.nombre}{Mozambique}
\@namedef{cf@extremo.pais.bot3.id}{MDG}
\@namedef{cf@extremo.pais.bot3.l2}{19.7}
\@namedef{cfa@extremo.pais.bot3.l2}{19.7}
\@namedef{cf@extremo.pais.bot3.nombre}{Madagascar}
\@namedef{cf@extremo.pais.n.max}{1}
\@namedef{cfa@extremo.pais.n.max}{1}
\@namedef{cf@extremo.pais.n.min}{1}
\@namedef{cfa@extremo.pais.n.min}{1}
\@namedef{cf@extremo.pais.top1.id}{SGP}
\@namedef{cf@extremo.pais.top1.l2}{64.2}
\@namedef{cfa@extremo.pais.top1.l2}{64.2}
\@namedef{cf@extremo.pais.top1.nombre}{Singapore}
\@namedef{cf@extremo.pais.top2.id}{LUX}
\@namedef{cf@extremo.pais.top2.l2}{63.5}
\@namedef{cfa@extremo.pais.top2.l2}{63.5}
\@namedef{cf@extremo.pais.top2.nombre}{Luxembourg}
\@namedef{cf@extremo.pais.top3.id}{GBR}
\@namedef{cf@extremo.pais.top3.l2}{54.9}
\@namedef{cfa@extremo.pais.top3.l2}{54.9}
\@namedef{cf@extremo.pais.top3.nombre}{the United Kingdom}
\@namedef{cf@gg.1.barrera_acceso.pct}{74.0}
\@namedef{cfa@gg.1.barrera_acceso.pct}{74.0}
\@namedef{cf@gg.1.barrera_confianza.pct}{51.6}
\@namedef{cfa@gg.1.barrera_confianza.pct}{51.6}
\@namedef{cf@gg.1.barrera_fisica.pct}{21.3}
\@namedef{cfa@gg.1.barrera_fisica.pct}{21.3}
\@namedef{cf@gg.1.barrera_responsabilidad.pct}{35.5}
\@namedef{cfa@gg.1.barrera_responsabilidad.pct}{35.5}
\@namedef{cf@gg.1.l2}{81.8}
\@namedef{cfa@gg.1.l2}{81.8}
\@namedef{cf@gg.2.barrera_acceso.pct}{64.2}
\@namedef{cfa@gg.2.barrera_acceso.pct}{64.2}
\@namedef{cf@gg.2.barrera_confianza.pct}{50.2}
\@namedef{cfa@gg.2.barrera_confianza.pct}{50.2}
\@namedef{cf@gg.2.barrera_fisica.pct}{33.0}
\@namedef{cfa@gg.2.barrera_fisica.pct}{33.0}
\@namedef{cf@gg.2.barrera_responsabilidad.pct}{44.8}
\@namedef{cfa@gg.2.barrera_responsabilidad.pct}{44.8}
\@namedef{cf@gg.2.l2}{69.9}
\@namedef{cfa@gg.2.l2}{69.9}
\@namedef{cf@gg.3.barrera_acceso.pct}{70.7}
\@namedef{cfa@gg.3.barrera_acceso.pct}{70.7}
\@namedef{cf@gg.3.barrera_confianza.pct}{37.7}
\@namedef{cfa@gg.3.barrera_confianza.pct}{37.7}
\@namedef{cf@gg.3.barrera_fisica.pct}{44.1}
\@namedef{cfa@gg.3.barrera_fisica.pct}{44.1}
\@namedef{cf@gg.3.barrera_responsabilidad.pct}{40.0}
\@namedef{cfa@gg.3.barrera_responsabilidad.pct}{40.0}
\@namedef{cf@gg.3.l2}{64.4}
\@namedef{cfa@gg.3.l2}{64.4}
\@namedef{cf@gg.4.barrera_acceso.pct}{69.6}
\@namedef{cfa@gg.4.barrera_acceso.pct}{69.6}
\@namedef{cf@gg.4.barrera_confianza.pct}{18.0}
\@namedef{cfa@gg.4.barrera_confianza.pct}{18.0}
\@namedef{cf@gg.4.barrera_fisica.pct}{35.4}
\@namedef{cfa@gg.4.barrera_fisica.pct}{35.4}
\@namedef{cf@gg.4.barrera_responsabilidad.pct}{10.8}
\@namedef{cfa@gg.4.barrera_responsabilidad.pct}{10.8}
\@namedef{cf@gg.4.l2}{78.3}
\@namedef{cfa@gg.4.l2}{78.3}
\@namedef{cf@gg.5.barrera_acceso.pct}{60.7}
\@namedef{cfa@gg.5.barrera_acceso.pct}{60.7}
\@namedef{cf@gg.5.barrera_confianza.pct}{43.8}
\@namedef{cfa@gg.5.barrera_confianza.pct}{43.8}
\@namedef{cf@gg.5.barrera_fisica.pct}{72.2}
\@namedef{cfa@gg.5.barrera_fisica.pct}{72.2}
\@namedef{cf@gg.5.barrera_responsabilidad.pct}{19.2}
\@namedef{cfa@gg.5.barrera_responsabilidad.pct}{19.2}
\@namedef{cf@gg.5.l2}{39.6}
\@namedef{cfa@gg.5.l2}{39.6}
\@namedef{cf@gg.6.barrera_acceso.pct}{61.8}
\@namedef{cfa@gg.6.barrera_acceso.pct}{61.8}
\@namedef{cf@gg.6.barrera_confianza.pct}{17.0}
\@namedef{cfa@gg.6.barrera_confianza.pct}{17.0}
\@namedef{cf@gg.6.barrera_fisica.pct}{90.3}
\@namedef{cfa@gg.6.barrera_fisica.pct}{90.3}
\@namedef{cf@gg.6.barrera_responsabilidad.pct}{26.6}
\@namedef{cfa@gg.6.barrera_responsabilidad.pct}{26.6}
\@namedef{cf@gg.6.l2}{17.4}
\@namedef{cfa@gg.6.l2}{17.4}
\@namedef{cf@gg.7.barrera_acceso.pct}{43.8}
\@namedef{cfa@gg.7.barrera_acceso.pct}{43.8}
\@namedef{cf@gg.7.barrera_confianza.pct}{7.6}
\@namedef{cfa@gg.7.barrera_confianza.pct}{7.6}
\@namedef{cf@gg.7.barrera_fisica.pct}{88.2}
\@namedef{cfa@gg.7.barrera_fisica.pct}{88.2}
\@namedef{cf@gg.7.barrera_responsabilidad.pct}{21.7}
\@namedef{cfa@gg.7.barrera_responsabilidad.pct}{21.7}
\@namedef{cf@gg.7.l2}{17.4}
\@namedef{cfa@gg.7.l2}{17.4}
\@namedef{cf@gg.8.barrera_acceso.pct}{66.4}
\@namedef{cfa@gg.8.barrera_acceso.pct}{66.4}
\@namedef{cf@gg.8.barrera_confianza.pct}{13.6}
\@namedef{cfa@gg.8.barrera_confianza.pct}{13.6}
\@namedef{cf@gg.8.barrera_fisica.pct}{86.0}
\@namedef{cfa@gg.8.barrera_fisica.pct}{86.0}
\@namedef{cf@gg.8.barrera_responsabilidad.pct}{29.5}
\@namedef{cfa@gg.8.barrera_responsabilidad.pct}{29.5}
\@namedef{cf@gg.8.l2}{18.4}
\@namedef{cfa@gg.8.l2}{18.4}
\@namedef{cf@gg.9.barrera_acceso.pct}{44.7}
\@namedef{cfa@gg.9.barrera_acceso.pct}{44.7}
\@namedef{cf@gg.9.barrera_confianza.pct}{10.9}
\@namedef{cfa@gg.9.barrera_confianza.pct}{10.9}
\@namedef{cf@gg.9.barrera_fisica.pct}{94.1}
\@namedef{cfa@gg.9.barrera_fisica.pct}{94.1}
\@namedef{cf@gg.9.barrera_responsabilidad.pct}{16.4}
\@namedef{cfa@gg.9.barrera_responsabilidad.pct}{16.4}
\@namedef{cf@gg.9.l2}{12.3}
\@namedef{cfa@gg.9.l2}{12.3}
\@namedef{cf@h1.dif.bajo_alto}{$-$23.06}
\@namedef{cfa@h1.dif.bajo_alto}{23.06}
\@namedef{cf@h1.dif.bajo_alto.p}{$<$0.001}
\@namedef{cfa@h1.dif.bajo_alto.p}{$<$0.001}
\@namedef{cfp@h1.dif.bajo_alto.p}{$p<0.001$}
\@namedef{cf@h1.dif.medio_alto_alto}{$-$10.57}
\@namedef{cfa@h1.dif.medio_alto_alto}{10.57}
\@namedef{cf@h1.dif.medio_alto_alto.p}{$<$0.001}
\@namedef{cfa@h1.dif.medio_alto_alto.p}{$<$0.001}
\@namedef{cfp@h1.dif.medio_alto_alto.p}{$p<0.001$}
\@namedef{cf@h1.dif.medio_bajo_alto}{$-$17.57}
\@namedef{cfa@h1.dif.medio_bajo_alto}{17.57}
\@namedef{cf@h1.dif.medio_bajo_alto.p}{$<$0.001}
\@namedef{cfa@h1.dif.medio_bajo_alto.p}{$<$0.001}
\@namedef{cfp@h1.dif.medio_bajo_alto.p}{$p<0.001$}
\@namedef{cf@h1.dummies.r2}{0.70}
\@namedef{cfa@h1.dummies.r2}{0.70}
\@namedef{cf@h1.n}{146}
\@namedef{cfa@h1.n}{146}
\@namedef{cf@h1.p}{$<$0.001}
\@namedef{cfa@h1.p}{$<$0.001}
\@namedef{cfp@h1.p}{$p<0.001$}
\@namedef{cf@h1.pendiente}{7.23}
\@namedef{cfa@h1.pendiente}{7.23}
\@namedef{cf@h1.pendiente.geih}{7.66}
\@namedef{cfa@h1.pendiente.geih}{7.66}
\@namedef{cf@h1.pendiente.hi}{7.8}
\@namedef{cfa@h1.pendiente.hi}{7.8}
\@namedef{cf@h1.pendiente.ic}{6.52 to 7.83}
\@namedef{cf@h1.pendiente.iguales}{7.43}
\@namedef{cfa@h1.pendiente.iguales}{7.43}
\@namedef{cf@h1.pendiente.lo}{6.5}
\@namedef{cfa@h1.pendiente.lo}{6.5}
\@namedef{cf@h1.pendiente.share}{4.2}
\@namedef{cfa@h1.pendiente.share}{4.2}
\@namedef{cf@h1.r2}{0.71}
\@namedef{cfa@h1.r2}{0.71}
\@namedef{cf@h1.se}{0.39}
\@namedef{cfa@h1.se}{0.39}
\@namedef{cf@h1.se.hc1}{0.47}
\@namedef{cfa@h1.se.hc1}{0.47}
\@namedef{cf@h2.b.bajo}{$-$0.81}
\@namedef{cfa@h2.b.bajo}{0.81}
\@namedef{cf@h2.b.bajo.p}{$<$0.001}
\@namedef{cfa@h2.b.bajo.p}{$<$0.001}
\@namedef{cfp@h2.b.bajo.p}{$p<0.001$}
\@namedef{cf@h2.b.medio_alto}{0.17}
\@namedef{cfa@h2.b.medio_alto}{0.17}
\@namedef{cf@h2.b.medio_alto.p}{0.086}
\@namedef{cfa@h2.b.medio_alto.p}{0.086}
\@namedef{cfp@h2.b.medio_alto.p}{$p=0.086$}
\@namedef{cf@h2.b.medio_bajo}{$-$0.06}
\@namedef{cfa@h2.b.medio_bajo}{0.06}
\@namedef{cf@h2.b.medio_bajo.p}{0.673}
\@namedef{cfa@h2.b.medio_bajo.p}{0.673}
\@namedef{cfp@h2.b.medio_bajo.p}{$p=0.673$}
\@namedef{cf@h2.brecha.medio}{0.06}
\@namedef{cfa@h2.brecha.medio}{0.06}
\@namedef{cf@h2.brecha.medio.p}{0.270}
\@namedef{cfa@h2.brecha.medio.p}{0.270}
\@namedef{cfp@h2.brecha.medio.p}{$p=0.270$}
\@namedef{cf@h2.n}{101}
\@namedef{cfa@h2.n}{101}
\@namedef{cf@h2.r.adi_uso}{0.86}
\@namedef{cfa@h2.r.adi_uso}{0.86}
\@namedef{cf@h3.n.aei}{426}
\@namedef{cfa@h3.n.aei}{426}
\@namedef{cf@h3.n.aei_tareas}{433}
\@namedef{cfa@h3.n.aei_tareas}{433}
\@namedef{cf@h3.n.eisfeldt}{432}
\@namedef{cfa@h3.n.eisfeldt}{432}
\@namedef{cf@h3.n.eloundou}{433}
\@namedef{cfa@h3.n.eloundou}{433}
\@namedef{cf@h3.n.eloundou_gpt4}{433}
\@namedef{cfa@h3.n.eloundou_gpt4}{433}
\@namedef{cf@h3.n.felten}{428}
\@namedef{cfa@h3.n.felten}{428}
\@namedef{cf@h3.n.webb_ai}{425}
\@namedef{cfa@h3.n.webb_ai}{425}
\@namedef{cf@h3.n.webb_robot}{425}
\@namedef{cfa@h3.n.webb_robot}{425}
\@namedef{cf@h3.n.webb_software}{425}
\@namedef{cfa@h3.n.webb_software}{425}
\@namedef{cf@h3.r.aei}{0.69}
\@namedef{cfa@h3.r.aei}{0.69}
\@namedef{cf@h3.r.aei_tareas}{0.69}
\@namedef{cfa@h3.r.aei_tareas}{0.69}
\@namedef{cf@h3.r.eisfeldt}{0.88}
\@namedef{cfa@h3.r.eisfeldt}{0.88}
\@namedef{cf@h3.r.eloundou}{0.93}
\@namedef{cfa@h3.r.eloundou}{0.93}
\@namedef{cf@h3.r.eloundou_gpt4}{0.93}
\@namedef{cfa@h3.r.eloundou_gpt4}{0.93}
\@namedef{cf@h3.r.felten}{0.89}
\@namedef{cfa@h3.r.felten}{0.89}
\@namedef{cf@h3.r.webb_ai}{0.11}
\@namedef{cfa@h3.r.webb_ai}{0.11}
\@namedef{cf@h3.r.webb_robot}{$-$0.74}
\@namedef{cfa@h3.r.webb_robot}{0.74}
\@namedef{cf@h3.r.webb_software}{$-$0.26}
\@namedef{cfa@h3.r.webb_software}{0.26}
\@namedef{cf@h3.rho.aei}{0.79}
\@namedef{cfa@h3.rho.aei}{0.79}
\@namedef{cf@h3.rho.aei_tareas}{0.77}
\@namedef{cfa@h3.rho.aei_tareas}{0.77}
\@namedef{cf@h3.rho.eisfeldt}{0.90}
\@namedef{cfa@h3.rho.eisfeldt}{0.90}
\@namedef{cf@h3.rho.eloundou}{0.95}
\@namedef{cfa@h3.rho.eloundou}{0.95}
\@namedef{cf@h3.rho.eloundou_gpt4}{0.95}
\@namedef{cfa@h3.rho.eloundou_gpt4}{0.95}
\@namedef{cf@h3.rho.felten}{0.88}
\@namedef{cfa@h3.rho.felten}{0.88}
\@namedef{cf@h3.rho.webb_ai}{0.11}
\@namedef{cfa@h3.rho.webb_ai}{0.11}
\@namedef{cf@h3.rho.webb_robot}{$-$0.74}
\@namedef{cfa@h3.rho.webb_robot}{0.74}
\@namedef{cf@h3.rho.webb_software}{$-$0.27}
\@namedef{cfa@h3.rho.webb_software}{0.27}
\@namedef{cf@h4.b1}{0.87}
\@namedef{cfa@h4.b1}{0.87}
\@namedef{cf@h4.b2}{$-$0.18}
\@namedef{cfa@h4.b2}{0.18}
\@namedef{cf@h4.n}{18,796}
\@namedef{cfa@h4.n}{18,796}
\@namedef{cf@h4.n.clusters}{923}
\@namedef{cfa@h4.n.clusters}{923}
\@namedef{cf@h4.p1}{$<$0.001}
\@namedef{cfa@h4.p1}{$<$0.001}
\@namedef{cfp@h4.p1}{$p<0.001$}
\@namedef{cf@h4.p2}{$<$0.001}
\@namedef{cfa@h4.p2}{$<$0.001}
\@namedef{cfp@h4.p2}{$p<0.001$}
\@namedef{cf@h4.pico.minutos}{11.8}
\@namedef{cfa@h4.pico.minutos}{11.8}
\@namedef{cf@humano.l2.pct}{45.7}
\@namedef{cfa@humano.l2.pct}{45.7}
\@namedef{cf@humano.l3.consenso.l2.n}{42}
\@namedef{cfa@humano.l3.consenso.l2.n}{42}
\@namedef{cf@humano.l3.n}{50}
\@namedef{cfa@humano.l3.n}{50}
\@namedef{cf@humano.nivel.media}{1.28}
\@namedef{cfa@humano.nivel.media}{1.28}
\@namedef{cf@modelo.l2.pct.humano}{36.67}
\@namedef{cfa@modelo.l2.pct.humano}{36.67}
\@namedef{cf@modelo.l2.pct.muestra}{37.33}
\@namedef{cfa@modelo.l2.pct.muestra}{37.33}
\@namedef{cf@modelo.nivel.media.humano}{1.03}
\@namedef{cfa@modelo.nivel.media.humano}{1.03}
\@namedef{cf@modelo.nivel.media.muestra}{1.03}
\@namedef{cfa@modelo.nivel.media.muestra}{1.03}
\@namedef{cf@n.fallos.haiku}{3}
\@namedef{cfa@n.fallos.haiku}{3}
\@namedef{cf@n.fallos.sonnet}{0}
\@namedef{cfa@n.fallos.sonnet}{0}
\@namedef{cf@n.humano}{300}
\@namedef{cfa@n.humano}{300}
\@namedef{cf@n.humano.hojas}{1}
\@namedef{cfa@n.humano.hojas}{1}
\@namedef{cf@n.modelos}{2}
\@namedef{cfa@n.modelos}{2}
\@namedef{cf@n.panel}{1,500}
\@namedef{cfa@n.panel}{1,500}
\@namedef{cf@n.panel.humano}{300}
\@namedef{cfa@n.panel.humano}{300}
\@namedef{cf@n.tareas.haiku}{18,793}
\@namedef{cfa@n.tareas.haiku}{18,793}
\@namedef{cf@n.tareas.sonnet}{18,796}
\@namedef{cfa@n.tareas.sonnet}{18,796}
\@namedef{cf@n.testretest}{100}
\@namedef{cfa@n.testretest}{100}
\@namedef{cf@n.validacion}{300}
\@namedef{cfa@n.validacion}{300}
\@namedef{cf@pais.BRA.l2}{39.9}
\@namedef{cfa@pais.BRA.l2}{39.9}
\@namedef{cf@pais.COL.l2}{38.3}
\@namedef{cfa@pais.COL.l2}{38.3}
\@namedef{cf@pais.IND.l2}{27.8}
\@namedef{cfa@pais.IND.l2}{27.8}
\@namedef{cf@pais.MEX.l2}{36.8}
\@namedef{cfa@pais.MEX.l2}{36.8}
\@namedef{cf@pais.USA.l2}{51.9}
\@namedef{cfa@pais.USA.l2}{51.9}
\@namedef{cf@panel.l2.pct}{42.9}
\@namedef{cfa@panel.l2.pct}{42.9}
\@namedef{cf@panel.nivel.media}{1.16}
\@namedef{cfa@panel.nivel.media}{1.16}
\@namedef{cf@placebo.h1.p}{$<$0.001}
\@namedef{cfa@placebo.h1.p}{$<$0.001}
\@namedef{cfp@placebo.h1.p}{$p<0.001$}
\@namedef{cf@placebo.p}{$<$0.001}
\@namedef{cfa@placebo.p}{$<$0.001}
\@namedef{cfp@placebo.p}{$p<0.001$}
\@namedef{cf@placebo.sd.media}{0.09}
\@namedef{cfa@placebo.sd.media}{0.09}
\@namedef{cf@placebo.sd.obs}{0.33}
\@namedef{cfa@placebo.sd.obs}{0.33}
\@namedef{cf@robustez.esco.cobertura.pct}{100.0}
\@namedef{cfa@robustez.esco.cobertura.pct}{100.0}
\@namedef{cf@robustez.esco.h1.n}{146}
\@namedef{cfa@robustez.esco.h1.n}{146}
\@namedef{cf@robustez.esco.h1.p}{$<$0.001}
\@namedef{cfa@robustez.esco.h1.p}{$<$0.001}
\@namedef{cfp@robustez.esco.h1.p}{$p<0.001$}
\@namedef{cf@robustez.esco.h1.pendiente}{4.66}
\@namedef{cfa@robustez.esco.h1.pendiente}{4.66}
\@namedef{cf@robustez.esco.h1.pendiente.gg6}{6.92}
\@namedef{cfa@robustez.esco.h1.pendiente.gg6}{6.92}
\@namedef{cf@robustez.esco.n.isco}{424}
\@namedef{cfa@robustez.esco.n.isco}{424}
\@namedef{cf@robustez.esco.n.isco.comun}{421}
\@namedef{cfa@robustez.esco.n.isco.comun}{421}
\@namedef{cf@robustez.esco.n.skills}{8,229}
\@namedef{cfa@robustez.esco.n.skills}{8,229}
\@namedef{cf@robustez.esco.r.isco}{0.88}
\@namedef{cfa@robustez.esco.r.isco}{0.88}
\@namedef{cf@robustez.esco.titular.l2}{38.0}
\@namedef{cfa@robustez.esco.titular.l2}{38.0}
\@namedef{cf@tareas.empates.pct}{32.5}
\@namedef{cfa@tareas.empates.pct}{32.5}
\@namedef{cf@tareas.l2.pct}{50.0}
\@namedef{cfa@tareas.l2.pct}{50.0}
\@namedef{cf@tareas.nivel0.pct}{25.9}
\@namedef{cfa@tareas.nivel0.pct}{25.9}
\@namedef{cf@tareas.nivel1.pct}{24.1}
\@namedef{cfa@tareas.nivel1.pct}{24.1}
\@namedef{cf@tareas.nivel2.pct}{47.6}
\@namedef{cfa@tareas.nivel2.pct}{47.6}
\@namedef{cf@tareas.nivel3.pct}{2.4}
\@namedef{cfa@tareas.nivel3.pct}{2.4}
\@namedef{cf@titular.global.l2}{35.2}
\@namedef{cfa@titular.global.l2}{35.2}
\@namedef{cf@titular.global.l2.geih}{35.6}
\@namedef{cfa@titular.global.l2.geih}{35.6}
\@namedef{cf@titular.global.l2.hi}{36.7}
\@namedef{cfa@titular.global.l2.hi}{36.7}
\@namedef{cf@titular.global.l2.iguales}{34.9}
\@namedef{cfa@titular.global.l2.iguales}{34.9}
\@namedef{cf@titular.global.l2.lo}{33.9}
\@namedef{cfa@titular.global.l2.lo}{33.9}
\@namedef{cf@titular.global.l2.pesos_uniformes}{38.6}
\@namedef{cfa@titular.global.l2.pesos_uniformes}{38.6}
\@namedef{cf@titular.global.l2.sin_imputados}{35.6}
\@namedef{cfa@titular.global.l2.sin_imputados}{35.6}
\@namedef{cf@titular.global.l2.sin_ponderar}{37.7}
\@namedef{cfa@titular.global.l2.sin_ponderar}{37.7}
\@namedef{cf@titular.global.l3}{2.5}
\@namedef{cfa@titular.global.l3}{2.5}
\@namedef{cf@titular.global.l3.geih}{2.5}
\@namedef{cfa@titular.global.l3.geih}{2.5}
\@namedef{cf@titular.global.l3.hi}{3.2}
\@namedef{cfa@titular.global.l3.hi}{3.2}
\@namedef{cf@titular.global.l3.iguales}{2.8}
\@namedef{cfa@titular.global.l3.iguales}{2.8}
\@namedef{cf@titular.global.l3.lo}{1.9}
\@namedef{cfa@titular.global.l3.lo}{1.9}
\@namedef{cf@titular.global.share}{29.5}
\@namedef{cfa@titular.global.share}{29.5}
\@namedef{cf@titular.global.share.hi}{30.3}
\@namedef{cfa@titular.global.share.hi}{30.3}
\@namedef{cf@titular.global.share.lo}{28.8}
\@namedef{cfa@titular.global.share.lo}{28.8}
\@namedef{cf@titular.ingreso.alto.l2}{48.7}
\@namedef{cfa@titular.ingreso.alto.l2}{48.7}
\@namedef{cf@titular.ingreso.alto.l3}{3.7}
\@namedef{cfa@titular.ingreso.alto.l3}{3.7}
\@namedef{cf@titular.ingreso.bajo.l2}{22.5}
\@namedef{cfa@titular.ingreso.bajo.l2}{22.5}
\@namedef{cf@titular.ingreso.bajo.l3}{1.1}
\@namedef{cfa@titular.ingreso.bajo.l3}{1.1}
\@namedef{cf@titular.ingreso.medio.l2}{31.0}
\@namedef{cfa@titular.ingreso.medio.l2}{31.0}
\@namedef{cf@titular.ingreso.medio.l3}{2.2}
\@namedef{cfa@titular.ingreso.medio.l3}{2.2}
\@namedef{cf@titular.ingreso.medio_alto.l2}{35.0}
\@namedef{cfa@titular.ingreso.medio_alto.l2}{35.0}
\@namedef{cf@titular.ingreso.medio_alto.l3}{2.7}
\@namedef{cfa@titular.ingreso.medio_alto.l3}{2.7}
\@namedef{cf@titular.ingreso.medio_bajo.l2}{28.3}
\@namedef{cfa@titular.ingreso.medio_bajo.l2}{28.3}
\@namedef{cf@titular.ingreso.medio_bajo.l3}{1.8}
\@namedef{cfa@titular.ingreso.medio_bajo.l3}{1.8}
\@namedef{cf@titular.modelo.haiku.l2}{51.4}
\@namedef{cfa@titular.modelo.haiku.l2}{51.4}
\@namedef{cf@titular.modelo.sonnet.l2}{35.3}
\@namedef{cfa@titular.modelo.sonnet.l2}{35.3}
\makeatother
\newif\ifsintetico
\sinteticofalse

